A residual-based non-orthogonality correction for force-balanced unstructured Volume-of-Fluid methods

Non-orthogonality errors in unstructured Finite Volume methods for simulating incompressible two-phase flows may break the force-balanced discretization. We show that applying the same explicit non-orthogonality correction for all gradient terms in the context of segregated solution algorithms is not sufficient to achieve force balance. To ensure force balance, we introduce a straightforward and deterministic residual-based control of the non-orthogonality correction, which removes the number of non-orthogonality corrections as a free parameter from the simulation. Our method is directly applicable to different unstructured finite-volume two-phase flow simulation methods as long as they discretize the one-field formulation of incompressible two-phase Navier-Stokes equations. We demonstrate force balance for the surface tension force and the gravity force near linear solver tolerance for an algebraic and a geometric Volume-of-Fluid method using the stationary droplet and stationary water column verification cases on polyhedral unstructured meshes with varying levels of non-orthogonality.

==> sections/high-density-ratios.tex <==
\section{Numerical methodology}
\label{sec:numerical-method-and-implementation}

\subsection{Single-field mass conservation and volume fraction conservation}\todo{Tomislav: revise}
\label{sec:Connection_mass_vof_transport}

Our goal is to compute the the cell centered density $\rho_c^{n+1}$ and the mass flux $\rho_f^o F_f^o$ necessary for discretizing \cref{eq:momentum-transport} using the second-order accurate collocated unstructured Finite Volume method \citep{Jasak1996, maric2014openfoam, moukalled2016finite}. The mass flux appears in the discretization of the single-field two-phase momentum convection term 
%
\begin{equation}
    \int_{\Omega_c} \nabla \cdot( \rho \v \otimes \v) \, dV
    = \int_{\partial \Omega_c} ( \rho \v \otimes \v) \cdot \n \, ds
    = \sum_{f \in F_c} \rho_f F_f \v_f + O_{\rho\v}(h^2).
    \label{eq:momterm}
\end{equation}
%

We first consider volume fraction advection. The volume fraction is defined using the phase-indicator \ref{eq:indicator} as
\begin{equation}
  \alpha_c(t) := \frac{1}{|\Cell{c}|}\int_{\Cell{c}} \chi(\x, t) \, dV.
  \label{eq:volfracdef}
\end{equation}
%
The volume fraction advection equation \cite{Maric2020}
%
\begin{equation}
    \frac{d}{dt}\int_{\Omega_c} \chi \, dV = |\Omega_c| \frac{d}{dt}\alpha_c(t) 
    = - \int_{\partial \Omega_c} \chi \v \cdot \n \, dS,
    \label{eq:alphaeqn1}
\end{equation}
%
 is equivalent to the advection equation for the phase $\Omega^+(t)$ indicated by $1 - \chi(\x,t)$, namely
%
\begin{equation}
    \frac{d}{dt}\int_{\Omega_c} (1 - \chi) \, dV = - |\Omega_c| \frac{d}{dt}\alpha_c(t) 
    =  -\int_{\partial \Omega_c} (1 - \chi) \v \cdot \n \, dS,
    \label{eq:alphaeqn2}
\end{equation}
%
since $\frac{d}{dt} \int_{\Omega_c} \, dV= 0$, as $\Omega_c\ne\Omega_c(t)$, and $\int_{\partial \Omega_c} \v\cdot \n \, dS = \int_{\Omega_c} \nabla \cdot \v \, dV = 0$ for incompressible two-phase flows without phase change. 

The mass conservation with single-field density \ref{eq:rhoindicator} in a fixed control volume $\Omega_c$ states
%
\begin{equation}
    \frac{d}{dt} \int_{\Omega_c} \rho \, dV = - \int_{\partial \Omega_c} \rho \v \cdot \n \, dS. \label{eq:massconserv}
\end{equation}
%
Inserting \cref{eq:rhoindicator} into the r.h.s. of \cref{eq:massconserv} and integrating over the time step $[\tn, \tnn]$ results in 
%
\begin{equation}
    \begin{aligned}
    % \rho_c^{n+1} & = 
    % \rho_c^n - \frac{1}{|\Omega_c|}\sum_{f \in F_c}
    % \left[
    %  \rho^- \int_{\tn}^{\tnn}\int_{S_f} \chi \v \cdot \n \, dS \, dt
    %  + \rho^ + \int_{\tn}^{\tnn}\int_{S_f} (1- \chi) \v \cdot \n \, dS \, dt
    % \right] \\
    & = \rho_c^n + \frac{1}{|\Omega_c|}
    \left[
     -\rho^-  \int_{\tn}^{\tnn}\sum_{f \in F_c}\int_{S_f} \chi \v \cdot \n \, dS \, dt
     - \rho^+  \int_{\tn}^{\tnn}\sum_{f \in F_c}\int_{S_f} (1 - \chi) \v \cdot \n \, dS \, dt,
    \right]
    \end{aligned}
    \label{eq:massintegral}
\end{equation}
% 
% which is also an exact equation, as $\partial \Omega_c = \bigcup_{f \in F_c} S_f$, where $S_f$ are non-linear surfaces that bound the control volume $\Omega_c$. 
Inserting the \cref{eq:alphaeqn1,eq:alphaeqn2} in the \cref{eq:massintegral} to replace the sums of surface integrals results in 
%
\begin{equation}
    \rho_c^{n+1} = \rho_c^n + \frac{\rho^-}{|\Omega_c|}|\Omega_c|\int_{\tn}^{\tnn}\frac{d}{dt}\alpha_c(t) \, dt
    + \frac{\rho^+}{|\Omega_c|}|\Omega_c|\int_{\tn}^{\tnn}-\frac{d}{dt}\alpha_c(t) \, dt, 
    \label{eq:rho-alpha-intermediate}
\end{equation}
leading finally to
%
\begin{equation}
    \rho_c^{n+1} = \rho_c^{n} + (\rho^- - \rho^+) (\alpha_c^{n+1} - \alpha_c^n).
    \label{eq:rho-alpha}
\end{equation}
%
\Cref{eq:rho-alpha} shows that solving \cref{eq:massconserv} for $\rho_c^{n+1}$ is equivalent to adding the solution of the volume fraction equation scaled with $(\rho^- - \rho^+)$ to $\rho_c^n$. 

Integrating the single-field density model (\ref{eq:rhoindicator}) over the control volume $\Omega_c$ gives
%
\begin{equation}
    \int_{\Omega_c} \rho \, dV = \int_{\Omega_c} \rho^-\chi + \rho^+(1 - \chi) \, dV.
    \label{eq:rhoindicatorintegral}
\end{equation}
%
Dividing \cref{eq:rhoindicatorintegral} by $|\Omega_c|$ results in the discrete single-field density model,
%
\begin{equation}
    \rho_c(t) = \rho^-\alpha_c(t) + \rho^+(1 - \alpha_c(t)),
    \label{eq:rhoalpha}
\end{equation}
%
which, evaluated at $\tnn$ and $\tn$ and subsequently subtracted, results in 
%
\begin{equation*}
    \begin{aligned}
   \rho_c^{n+1} - \rho_c^n &= \rho^-\alpha_c^{n+1} + \rho^+(1 - \alpha_c^{n+1}) - 
   \rho^-\alpha_c^n - \rho^+(1 - \alpha_c^n) \\
   & = (\rho^- - \rho^+)(\alpha_c^{n+1} - \alpha_c^n),
   \end{aligned}
   \end{equation*}
%
which is \cref{eq:rho-alpha}: solving the volume fraction advection equation \cref{eq:alphaeqn1} and using the single-field density model to compute the cell centered density by \cref{eq:rhoindicator} is equivalent to solving the mass conservation equation (\ref{eq:massconserv}).
%In other words, solving the volume fraction equation for $\alpha_c^{n+1}$ and using the single-field density model \cref{eq:rhoalpha} to compute the cell-centered density $\rho_c^{n+1}$ is equivalent to solving the mass conservation equation (\ref{eq:massconserv}) for $\rho_c^{n+1}$.

Note that all equations above are exact, as $\partial \Omega_c := \bigcup_{f \in F_c} S_f$, where $S_f$ are non-linear surfaces that bound the control volume $\Omega_c$, and the temporal integration of a temporal derivative over a fixed time interval is exact by the fundamental theorem of calculus. 

\citet{Ghods2013} introduce the auxiliary mass conservation equation as a means for ensuring the consistency of the two-phase momentum convection, and in \cite{Liu2021} we provide the theoretical reasoning for the auxiliary mass conservation equation. Contrary to \citet{Ghods2013}, \cref{eq:rho-alpha} and  \cref{eq:rhoindicatorintegral} both demonstrate, that the solution of the volume fraction equation in the context of the VOF method is exactly equivalent to the solution of the auxiliary mass conservation equation. Consequentially, flux-based VOF methods are inherently consistently handling high density ratios on the level of the mathematical model. This seems to render the auxiliary mass conservation equation unnecessary for the VOF method. 
% that ensures the consistency between \cref{eq:rhoalpha} and \cref{eq:rho-alpha}. 

% It is crucial to note, that we have not used any approximations for evaluating the integrals specific to the update of cell-centered quantities, thus far. This makes the derived equivalence between the $\alpha_c^{n+1}$ and the $\rho_c^{n+1}$ update valid for any VOF method. Specific VOF methods used to compute $\alpha_c^{n+1}$ introduce specific errors on the r.h.s. of \cref{eq:rho-alpha}, however, this does not impact the equality in \cref{eq:rho-alpha} (or its meaning), it only adds a numerical error on the r.h.s., which is expected by any numerical method.

% We have shown in \citep{Liu2021}, that the numerical consistency of the single-field two-phase momentum convection is based on updating the cell-centered density $\rho_c^{n+1}$ by solving a mass conservation equation, \emph{or its equivalent}. This condition is not fulfilled by the Level Set method, Front Tracking method or their hybrids. As the VOF method solves \cref{eq:alphaeqn1}, and we show here that this \emph{is equivalent} to solving the mass conservation equation for the single-field density $\rho$, VOF method $\alpha_c(t)$ advection \emph{is equivalent} to the solution of the mass conservation equation for $\rho$. 

However, the following question arises: if flux-based VOF methods by construction ensure numerical stability for the two-phase momentum convection with high density ratios, where do the numerical inconsistencies reported throughout the literature for the VOF method \citep{fuster2018,Zuzio2020,Pal2021,Arrufat2021,Liu2022,Jin2022} come from? 

Although \cref{eq:rho-alpha} demonstrates an important equivalence for the VOF methods in the mathematical model, it does not contain any information about how $\alpha_c^{n+1}$ is computed discretely - this will depend on the type of the VOF method. 

If we use a second-order accurate flux-based VOF method, the approximations applied to the temporal and surface integrals for the fluxed phase-specific volumes $V_f^\alpha$ when solving \cref{eq:alphaeqn1} lead to
%
\begin{equation}
    \alpha_c^{n+1} = \alpha_c^n - \frac{1}{|\Omega_c|} \sum_{f \in F_c} \int_{\tn}^{\tnn}\int_{S_f} \chi \v \cdot \n \, dS \, dt
    = \alpha_c^n + \frac{1}{|\Omega_c|}\sum_{f \in F_c} |V_f^\alpha|_s
    + O_\alpha(\Delta t^p) + O_\alpha(h^2).
    \label{eq:alpha-discrete}
\end{equation}
%
Note that 
\begin{equation}
    |V_f^\alpha|_s = sgn(F_f)|V_f^\alpha|
\end{equation}
is a signed magnitude of a geometrically approximated phase-specific volume $V_f^\alpha$ \citep{Maric2020}, whose sign is determined by the face-centered volumetric flux 
\begin{equation}
    F_f := \v_f \cdot \Sf,
\end{equation}
where $\v_f$ is the second-order accurate face-centered velocity average and $\Sf$ is the surface area-normal vector oriented outwards of $\partial \Omega_c$.



Spatially second-order accurate flux-based VOF methods make it possible to compute $\rho_f F_f$ using \cref{eq:rho-alpha} and \cref{eq:alpha-discrete}.
Reordering \cref{eq:alpha-discrete}, results in 
%
\begin{equation}
     \alpha_c^{n+1} - \alpha_c^n = \frac{1}{|\Omega_c|}\sum_{f \in F_c}  |V_f^\alpha|_s
      + O_\alpha(\Delta t^p) + O_\alpha(h^2)
    \label{eq:alpha-diff}
\end{equation}
%
Inserting \cref{eq:alpha-diff} into \cref{eq:rho-alpha} results in 
%
\begin{equation}
    \rho_c^{n+1} - \rho_c^{n} = \frac{\rho^- - \rho^+}{|\Omega_c|} \sum_{f \in F_c} |V_f^\alpha|_s + (\rho^- - \rho^+)[O_\alpha(\Delta t^p) + O_\alpha(h^2)]
    \label{eq:rhodiffvfalpha}
\end{equation}\todo{Tomislav: this is already giving a mathematically consistent $\rho_c^{n+1}$. However, this also shows we cannot affort any overshoots and undershoots in alpha, we might get negative densities. Also what to do about the mass flux?}
%
% The difference $\rho_c^{n+1} - \rho_c^n$ in \cref{eq:rhodiffvfalpha} can be expressed by integrating \cref{eq:massconserv} over $[\tn, \tnn]$, resulting in 
% %
% \begin{equation}
%     \frac{1}{|\Omega_c|}\sum_{f \in F_c}\int_{\tn}^{\tnn} \rho_f F_f \, dt =  \frac{\rho^- - \rho^+}{|\Omega_c|} \sum_{f \in F_c} |V_f^\alpha|_s + (\rho^- - \rho^+)[O_\alpha(\Delta t^p) + O_\alpha(h^2)],
%     \label{eq:rhofvfalpha}
% \end{equation}
% % 
% and after temporal integration,  
% %
% \begin{equation}
%     \sum_{f \in F_c} |M_f|_s + O_\rho(\Delta t^l) + O_\rho(h^2) =  (\rho^- - \rho^+) \sum_{f \in F_c} |V_f^\alpha|_s + (\rho^- - \rho^+)[O_\alpha(\Delta t^p) + O_\alpha(h^2)],
%     \label{eq:mfvfalpha}
% \end{equation}
% %
% similar to the integral relations derived by \citet[sec 3.4.1]{Arrufat2021}, with the significant difference of not separating the face-centered density from the integral value, and generalizing the fluxed phase-specific volume $V_f^\alpha$. As \citet{Arrufat2021} point out, integrals complicate the computation of $\rho_f F_f$ from the integral value $|V_f^\alpha|_s$.
% Furthermore, \cref{eq:mfvfalpha} shows that the numerical consistency on the discrete level, expected by the exact equation \cref{eq:rho-alpha}, depends on the cancellation of the errors in discretely computing the mass $M_f$ fluxed over each $S_f$, and errors in computing the fluxed phase-specific volume $V_f^\alpha$, scaled by $(\rho^- - \rho^+)$. 
% In other words, if the $O_\rho$ errors do not exactly cancel out with the $O_\alpha$ errors multiplied by $(\rho^- - \rho^+)$ in \cref{eq:mfvfalpha}, the consistency enforced by the mathematical model in \cref{eq:rho-alpha} will not be satisfied on the discrete level. Moreover, \cref{eq:mfvfalpha} shows that any remainder of a failed cancellation will be multiplied with $(\rho^- - \rho^+)$, and scale with the density difference leading to catastrophic failures with high density ratios, as demonstrated in the results section. For methods that do not solve a volume fraction equation, error cancellation can be ensured by actually solving an auxilliary mass conservation equation for $\rho_c^{n+1}$ introduced by \citet{Hermann}\todo{Jun:citation}, but using a phase-specific volumetric flux geometrically approximated from whatever approximation is available  of the fluid interface $\Sigma(t)$, as we did for the Level Set / Front Tracking method in \citep{Liu2021}. For flux-based VOF methods which solve a volume fraction equation, error cancellation in \cref{eq:mfvfalpha} is ensured. Spatial second-order error resulting from face-centered averaging cancels because 
% %
% \begin{equation}
%     \frac{1}{|S_f|}\int_{S_f} \rho \, dS 
%     = \frac{1}{|S_f|}\int_{S_f} \rho \, dS
% \end{equation}


% is achieved by computing the mass flux $\rho_f F_f$ from the fluxed phase-specific volume $|V_f^\alpha|_s$ integrated as a part of the solution of the volume fraction advection equation. 

The consistency of the mass flux calculated from the scaled phase-specific volume can be demonstrated for a simplified Euler temporal integration of $|V_f^\alpha|_s$, namely
%
\begin{equation}
\begin{aligned}
    |V_f^\alpha|_s^{Euler}  & = \int_{\tn}^{\tnn} \int_{S_f} \chi \v \cdot \n \, dS \, dt 
    = \frac{F_f^n}{|S_f|} \int_{\tn}^{\tnn} \int_{S_f} \chi \, dS, dt  + O_\alpha(\Delta t) + O_\alpha(h^2) \\
    & = F_f^n \int_{\tn}^{\tnn} \alpha_f(t) \, dt + O_\alpha(\Delta t) + O_\alpha(h^2) \\
    & = F_f^n \alpha_f^n \Delta t + O_\alpha(\Delta t) + O_\alpha(h^2).
\end{aligned}
  \label{eq:vfalphaeuler}
\end{equation}
%
Multiplying \cref{eq:vfalphaeuler} with $(\rho^-  - \rho^+)$ We emphasize that \cref{eq:vfalphaeuler} is a simplified scheme used here to derive the discrete mass-flux consistency condition, it is not a practically usable scheme for advecting $\alpha_c$, because it is significantly less accurate than modern geometrical schemes \citep{Maric2020}.

Multiplying  $|V_f^\alpha|_s^{Euler}$ from \cref{eq:vfalphaeuler} with $(\rho^- - \rho^+)$, instead of actually integrating $\rho_f F_f$ over $[\tn, \tnn]$ to obtain $|M_f|_s$ ensures the consistency in \cref{eq:rhofvfalpha} 
\begin{equation}
\begin{aligned}
    \int_{\tn}^{\tnn} \rho_f F_f dt = \frac{(\rho^- - \rho^+)|V_f^\alpha|_s^{Euler}}{\Delta t} =  (\rho^- - \rho^+)F_f^n \alpha_f^n + (\rho^- - \rho^+)(O_\alpha(\Delta t) + O_\alpha(h^2)).
\end{aligned}
  \label{eq:vfalphaeuler}
\end{equation}


applied on the integrals in \cref{eq:rhofvfalpha}, we can check  cancellation of $O_\rho$ and the scaled $O_\alpha$ is ensured since
%
\begin{equation}
        \sum_{f \in F_c}\rho_f^n F_f^n \Delta t = (\rho^- - \rho^+)\sum_{f \in F_c} |V_f^\alpha|_s^{Euler},
        \label{eq:EulerBalance}
\end{equation}
%
where $|V_f^\alpha|_s^{Euler}$ integrated, say, using the isoAdvector scheme \citep{Roenby2016} as
\begin{equation}
|V_f^\alpha|_s^{Euler}  = F_f^n \int_{\tn}^{\tnn} \int_{S_f} \chi(\x,t) \, dS \, dt,
\label{eq:isoadveuler}
\end{equation}
with the submerged area integral computed exactly by moving the piecewise-linear interface in the upwind cell using the Euler displacement $\v_c \Delta t$. The Euler temporal integration of the integral on the r.h.s. of \cref{eq:isoadveuler} makes it possible to consistently compute the mass flux by scaling the phase-specific fluxed volume 
%
\begin{equation}
    \rho_f^n F_f^n = \dfrac{(\rho^- - \rho^+)|V_f^\alpha|_s}{\Delta t}.
    \label{eq:massfluxvfalphaeuler}
\end{equation}
%
The same consistency would be ensured if $V_f^\alpha$ would be constructed using a flux-based VOF method that maps $S_f$ using the reverse flow-map (e.g., \citep{Maric2018}). In other words, if $V_f^\alpha$ is constructed geometrically using displacements given by $\v(\x,t^n)\Delta_t$, regardless of the geometrical approximation, $V_f^\alpha$ is constructed using displacements constant over $\Delta_t$, so dividing the volume $V_f^\alpha$ with $\Delta_t$ exactly results in the volumetric flux that corresponds to Euler temporal integration scheme.

However, if the Crank-Nicolson scheme is applied for the mass conservation equation, 
%
\begin{equation}
        \sum_{f \in F_c}0.5 \Delta t (\rho_f^{n+1} F_f^{n+1} + \rho_f^n F_f^n) = (\rho^- - \rho^+)\sum_{f \in F_c} |V_f^\alpha|^{CN},
        \label{eq:massfluxvfalphacn}
\end{equation}
% 
there is an issue in evaluating the mass flux from $|V_f^\alpha|^{CN}$. Namely, the Crank-Nicolson scheme involves $\rho_f F_f$ at $\tn$ and $\tnn$ in the same equation, making it impossible to express either one without the other, using $|V_f^\alpha|^{CN}$.
Specifically, from \cref{eq:massfluxvfalphacn}, we could compute the mass flux at $\tnn$ as 
\begin{equation}
        \rho_f^{n+1} F_f^{n+1} = \frac{2(\rho^- - \rho^+)|V_f^\alpha|^{CN}}{\Delta t} - \rho_f^n F_f^n
        \label{eq:CNDiscretization}
\end{equation}
% 
This confirms the difficulty in evaluating mass flux density from the integrals that appear in \cref{eq:rhofvfalpha} pointed out by \citet{Arrufat2021}.
Furthermore, in order to integrate $|V_f^\alpha|$ using the Crank-Nicolson scheme (i.e.\ trapezoidal quadrature), the position of the interface at $\tnn$ must be known, namely $\Sigma^{n+1}$. 
The interface $\Sigma^{n+1}$ can be computed by forward extrapolation in time \cite{Roenby2016}, however, this kind of quadrature does not exactly correspond to the Crank-Nicolson scheme used in the momentum equation, because the extrapolation of the interface $\Sigma^{n+1}$ used old-time velocities $\v_c^{m}, m \le n$, and Crank-Nicolson in the momentum equation uses the new time-step velocity $\v_c^{n+1}$. 

An entirely different form of inconsistency arises when $\rho_f F_f$ is additionally altered in the $p-\v$ coupling, e.g. by applying flux limiting schemes. This changes the relation of the mass flux $\rho_f F_f$ to $|V_f^\alpha|$, even if $\rho_f F_f$ was originally consistently calculated from $|V_f^\alpha|$.\todo{Discuss the details in zoom.}

If, however, one does not integrate \cref{eq:massconserv} and \cref{eq:alphaeqn1} in time, then it becomes clear that the mass flux $\rho_f F_f$ is uniquely determined by $\chi(\x,t)$ \citep{Liu2021}, however, this requires an introduction of an auxiliary mass conservation equation \cite{Ghods2013}, and the cell-centered density that is only used for the $p-\v$ coupling.

From \cite{}, at any time $t$,\todo{Discuss: does this connect with getRhoPhi in isoAdvection?}
%
\begin{equation}
    \rho_f F_f = \rho^- \alpha_f F_f + \rho^+(1 - \alpha_f)F_f
    = \rho^- \alpha_f F_f + \rho^+F_f - \rho^+\alpha_fF_f
    = (\rho^- - \rho^+)\alpha_f F_f + \rho^+F_f
\end{equation}
%

\subsection{Solution algorithm in interIsoRhoFoam} \label{sec:introduction_solver}
%% brief intro of interIsoFoam, algorithm summary chart, new features of interIsoRhoFoam, isoadvector Johan2016, enriched reconstruction scheme Henning2019
\citet{Roenby2016} devised a novel geometric VOF interface advection method named isoAdvector and implemented this method by modifying widely used two-phase flow solver interFoam in the \OF  platform. The modified solver is called interIsoFoam. Different from the algebraic compressive method in interFoam, which adopts a special limiter, i.e. MULES (Multidimensional Universal Limiter with Explicit Solution), to correct the flux transport of the phase indicator in each cell to ensure the sharpness and boundedness \citep{Damian2013}, isoAdvector in interIsoFoam reconstructs the interfaces, and calculates the transport of one fluid's volume cross the cell faces at a time step to evolve the interfaces, as well as the volume fraction. \citet{Scheufler2019} enhanced the isoAdvector's interface reconstruction scheme. Two iterative variations of the RDF (Reconstructed Distance Function) scheme, namely iso-RDF and plic-RDF, were suggested and implemented in interIsoFoam as scheme selection alternatives. Various comparisons between isoAdvector and other methods show the interIsoFoam's good performances of surface sharpness, volume fraction boundedness, and mass conservation \cite{Roenby2016, Olsson2017, Larsen2019}. Hence, we built our consistent solution method based on the interIsoFoam and named the modified one interIsoRhoFoam to distinguish these two solvers. 

In \citep{Liu2021}, we propounded that discretizing an auxiliary mass conservation equation consistently with momentum equation plays a key role in stabilizing and converging numerical error caused by the high density ratio of two-phase flows. To integrate the consistent property to interIsoFoam, an auxiliary mass advection equation in conservative form is resolved after advancing the interface with isoAdvector method. The auxiliary mass equation has the form:

%%
\begin{equation}
    \partial_t \rho + \nabla \cdot(\rho\v) = 0,
    \label{eq:mass-transport}
\end{equation}
%%

For the clarification, we consider our consistent method exemplified by the Euler discretization in an iteration step:

%%
\begin{equation}
    \rho^{m+1}_c = \rho^m_c + \frac{\Delta t}{|V_{\Cell{c}}|}\sum_f \rho^{m+1}_f F^m_f, \quad F^m_f = \v_f^m \cdot \Sf,
    \label{eq:rho_update_Euler}
\end{equation}
%%

where the $F_f$ indicates the volumetric flux across the cell face $f$, the superscript $m$ denotes the iteration step in the pressure-velocity coupling algorithm, that ranges from $n$ to $n+1$. 

A novelty of the \rhoLENT method \citep{Liu2021} is that we revealed the restriction of relationship between the phase indicator and the face-centered density $\rho_f$, based on the principle of mass conservation. Following the restriction, the surface integrals of mass flux at time step $n+1$ is expressed in the form of

%%
\begin{equation}
    \int_{\partial \Omega_c} \rho^{m+1} \v^m \cdot \n dS = 
        \int_{\partial \Omega_c} [\rho^- \chi^{m+1} + \rho^+(1 - \chi^{m+1})] \v^m \cdot \n \, dS,
\end{equation}
%%

then discretized 

%%
\begin{equation}
    \begin{aligned}
        \sum_{f \in F_c} \rho_f^{m+1} F_f^m 
        & = 
        \sum_{f \in F_c} 
            \left[
                \rho^- \alpha_f^{m+1} 
                + \rho^+ (1 - \alpha_f^{m+1})
            \right] F_f^m, 
    \end{aligned}
    \label{eq:rhodiscreteflux}
\end{equation}
%%

where, accordingly, 

%%
\begin{equation}
    \alpha_f^{m+1} := \frac{1}{|S_f|}\int_{S_f} \chi^{m+1} \, dS 
    \equiv \dfrac{|\Omega^-(t^{m+1}) \cap S_f|}{|S_f|}
    \label{eq:update_alpha_f}
\end{equation} 
%%

is the ratio of cell face area submerged in $\Omega^-(t^{m+1})$ to the whole face area $|S_f|$, which is called area fraction for brevity later, and 

%%
\begin{equation}
    \rho_f^{m+1} = \rho^-\alpha_f^{m+1} + \rho^+(1-\alpha_f^{m+1})
    \label{eq:update_rho_f}
\end{equation}
%%

is the face-centered density. 
  
The identical temporal and spatial scheme are exploited to discretize the momentum advection equation. The discretized momentum equation is represented by 

%%
\begin{equation}
    \rho^{m+1}_c \v^{m+1} - \rho^m_c \v^m + \frac{\Delta t}{|V_{\Cell{c}}|}\sum_f \rho^{m+1}_f F^m_f \v_f^{m+1} = \frac{\Delta t}{|V_{\Cell{c}}|} \cdot RHS^{m+1},
    \label{eq:rhov_update_Euler}
\end{equation}
%%

in which $\rho^{m+1}_c$ and $\rho^{m+1}_f F^m_f$ are known and consistent with the values in \cref{eq:rho_update_Euler}.  
 
%%
\begin{center}
\begin{algorithm}[H]
    \centering
    \caption{The solution algorithm in interIsoRhoFoam.}
    \label{alg:interIsoRho}
    {\small
    \centering
    \begin{algorithmic}[1]
        \While{simulation time $\le$ end time}
        \While{$p-\v$ coupling}
            \State Advect the interface to $\tilde{\Sigma}^{m+1}$ using isoAdvector method. \Comment \citep{Roenby2016, Scheufler2019}
%             \State Compute the signed-distance field $\phi^{n+1}$ from $\tilde{\Sigma}^{n+1}$ at $\x_c, \x_f, \x_p$ in the narrow-band. \Comment \cite{maric2015lentfoam}
%             \State Compute $\alpha_c^{n+1}$ from $\phi_c^{n+1},\phi_p^{n+1}$. \Comment \cite{tolle2020saample}
            \State Compute the area fraction $\alpha_f^{m+1}$ from the ratio of the submerged cell face area to the whole cell face area . \Comment \Cref{eq:update_alpha_f}
            \State Compute the face-centered densities $\rho_f^{m+1}$ using $\alpha_f^{n+1}$.  \Comment \Cref{eq:update_rho_f}
            \State Solve the continuity equation using $\rho_f^{m+1}F_f^m$ for cell-centered densities $\rho_c^{m+1}$.   \Comment \Cref{eq:rho_update_Euler}
            \State Use $\rho_c^{m+1}$ and $\rho_f^{m+1}F_f^m$ in the discritized momentum transport equation to compute $\v_c^{m+1}, F_f^{m+1}$. 
            
            \Comment \citep{Liu2021} and \cref{eq:rhov_update_Euler}
            \EndWhile
            \State Make $\rho_c^{n+1}$ consistent with $\tilde{\Sigma}^{n+1}$, i.e.\ $\rho_c^{n+1}=\alpha_c^{n+1}\rho^-+(1-\alpha_c^{n+1})\rho^+$.
            \State Make $\mu_c^{n+1}$ consistent with $\tilde{\Sigma}^{n+1}$, i.e. $\mu_c^{n+1}:=\alpha_c^{n+1}\rho^-\nu^-+(1-\alpha_c^{n+1})\rho^+\nu^+$.
        \EndWhile
    \end{algorithmic}
    }
\end{algorithm}
\end{center}
%%

% \subsubsection{temporal scheme}
%% briefly introduct euler schme and CrankNicolson scheme

% \subsubsection{spatial scheme for the convective term}
%% explain why we use upwind scheme 


%%
\subsection{Submerged interface cell face area fraction}
\label{sec:submerged_areaFraction}
% subalgorithm for caculating alphaf 

%
\begin{figure}[!htb]
    \begin{subfigure}[t]{.49\textwidth}
    \centering
    \def\svgwidth{.96\linewidth}
    \input{figures/cuttedCell.pdf_tex}
    \caption{Neighbor cells intersected with PLIC interfaces.}
    \label{fig:cuttedCell}
   \end{subfigure} \hfill
    \begin{subfigure}[t]{.49\textwidth}
    \centering
    \def\svgwidth{.96\linewidth}
    \input{figures/cuttedArea.pdf_tex}
    \caption{Faces intersected with downwind (D) and upwind (U) PLIC interfaces.}
    \label{fig:cuttedArea}
   \end{subfigure} 
   \caption{The interface reconstruction in two adjcent cells. Green faces: interfaces; Red points: intersection points; Blue lines: intersection line segment. Subscript $U$: Upwind cell; Subscript $D$: Downwind cell .}
   \label{fig:reconstructedInterface}
\end{figure}
%

% the $F^m_f$ indicates the volumetric flux across the cell face $f$ and is updated iteratively to $F^{n+1}_f$ in the pressure-velocity coupling algorithm. 
The signed distances of the face vertices are weighted in the \rhoLENT method to evaluate the area fraction\citep{Liu2021}. In a geometric VOF method, the reconstructed interfaces' information, such as the intersection points and the intersection line segments of interfaces and cell faces as depicted by the red dots and the blue line segments in \cref{fig:reconstructedInterface}, are available, which results that the calculation of the area fraction is intuitive to be implemented from \cref{eq:update_alpha_f}. It's worth mentioning that the line segments, which are the intersection of the piecewise interfaces and the shared face of two adjacent interface cells, as shown in \cref{fig:cuttedCell}, usually are not collinear. The \cref{fig:cuttedArea} shows closely that there are two intersection line segments on a cell face. The intersection line segment of the interface and the upwind cell are selected as the submerged area border to calculate the area fraction. The entire  algorithm of $\alpha_f^{m+1}$ evaluation is demonstrated in \cref{alg:calc_alphaf}. To differentiate two cells connected by a shared cell face, we refer to one as the owner cell and the other as the neighbor cell.   
 
%%
\begin{center}
\begin{algorithm}[H]
    \centering
    \caption{The sub-algorithm of calculating the face-centred area $\alpha_f$ on unstructured grids.}
    \label{alg:calc_alphaf}
    {\small
    \centering
    \begin{algorithmic}[1]
        \State Initialize $\rho_f^{m+1}$, $\alpha_f^{m+1}$ with the upwind cell value $\rho_U^{m}$, $\alpha_U^{m}$.
        \State Advect the interface to $\tilde{\Sigma}^{m+1}$ using isoAdvector method. \Comment \citep{Roenby2016, Scheufler2019}
        \For{Cell face $j$}
            \If{Volume flux $\phi_j>0$}
                \If{Owner cell of face $j$ is a surface cell}
                \State Utilize interface in the owner cell to update $\alpha_f^{m+1}$. \Comment \Cref{eq:update_alpha_f}
                \EndIf
            \Else 
                \If{Neighbor cell of face $j$ is a surface cell}
                \State Utilize interface in the neighbor cell to update $\alpha_f^{m+1}$. \Comment \Cref{eq:update_alpha_f}
                \EndIf
            \EndIf
        \EndFor
        \State Update $\rho_f^{m+1}$, \ $\rho_f^{m+1}=\alpha_f^{m+1}\rho^-+(1-\alpha_f^{m+1})\rho^+$.
        \State Update $\mu_f^{m+1}$, $\mu_f^{m+1}:=\alpha_f^{m+1}\rho^-\nu^-+(1-\alpha_f^{m+1})\rho^+\nu^+$.
    \end{algorithmic}
    }
\end{algorithm}
\end{center}
%%
